An Axiomatic Approach to Detect Information Leaks in Concurrent Programs

Realizing flow security in a concurrent environment is extremely challenging, primarily due to non-deterministic nature of execution. The difficulty is further exacerbated from a security angle if sequential threads disclose control locations through publicly observable statements like print, sleep, delay, etc. Such observations lead to internal and external timing attacks. Inspired by previous works that use classical Hoare style proof systems for establishing correctness of distributed (real-time) programs, in this paper, we describe a method for finding information leaks in concurrent programs through the introduction of leaky assertions at observable program points. Specifying leaky assertions akin to classic assertions, we demonstrate how information leaks can be detected in a concurrent context. To our knowledge, this is the first such work that enables integration of different notions of non-interference used in functional and security context. While the approach is sound and relatively complete in the classic sense, it enables the use of algorithmic techniques that enable programmers to come up with leaky assertions that enable checking for information leaks in sensitive applications.

==> statemachine.tex <==
\section{Information Flow State Machine}
\label{sec:state_machine}
In this section,  we describe the information flow state machine on which we can drape the formal definition of a generalized notion of non-interference for sequential and concurrent programs.

\begin{defn}[\textbf{State Machine} $\mathbf{\mathcal{M}}$]
A state machine $\mathcal{M}$ is defined as a transition system $(\mathcal{Q},\mathcal{U},\mathcal{C},\delta)$, where $\mathcal{Q}$ represent the set of states in the system, $\mathcal{U}$ denote the set of users, $\mathcal{C}$ denote the set of commands of the machine, and $\delta:\mathcal{Q}\times\mathcal{U}\times\mathcal{C}\rightarrow\mathcal{Q}$ denote the state transition function.
\end{defn}

For the purpose of this paper, we consider the set of states $\mathcal{Q}$ to be defined as $\mathcal{Q}=2^{(\mathcal{U}\times\mathcal{V})}$. Then a state $q\in\mathcal{Q}$ is a finite set of tuples $(u,v)$, where $u\in\mathcal{U}$ is a user or process and $v\in\mathcal{V}$ is a variable or memory location. Further, we consider that the function $\lambda$ implicitly maps each user $u$ and variable $v$ to its respective security label $\underline{u}$ and $\underline{v}$ from the lattice $\mathcal{L}$, i.e., $\lambda:\mathcal{U}\times\mathcal{V}\rightarrow\mathcal{L}$. Similarly, the function $\gamma$ implicitly maps a variable $v$ to its value $\bar{v}$ from a semantic domain of values denoted by $V$, i.e., $\gamma:\mathcal{V}\rightarrow V$.

\begin{defn}[\textbf{Execution}]
For a given state machine $\mathcal{M}$ and a command $c$ issued by the user $u$, the detailed process by which a given initial state $q$ is changed to $\delta(q,u,c)$ is referred as an execution of $c$ in $q$ by user $u$.
\end{defn}

While instantiating the state machine for program computation, execution of a given command $c$ (or program statement) in a state $q$ issued by the user (or process) $u$ involves a series of steps such as decomposing the command into an input sequence of primitive operations such as read or write the variable and corresponding state transitions, checking access permission for each operation, and finally allow or deny based on the given information flow policy. For this instance, let us assume that the users have the required access permissions for the variables and restrict our attention to the first and last steps only. Let $r$ denote read and $w$ denote write, and $\mathcal{A}=\{r,w\}$ denote the set of all possible primitive operations. Then $(\mathcal{V}\times\mathcal{A})^\ast$ denote the set of all possible finite input sequences. For an input sequence $s\in(\mathcal{V}\times\mathcal{A})^\ast$, $|s|$ denote the length of $s$, and for $1\leq i \leq |s|$, $s_i$ denote the $i^{th}$ element in $s$.

\begin{defn}[\textbf{Input Sequence of an Execution}]
For a state machine $\mathcal{M}$, an input sequence corresponding to an execution of the command $c$ is defined as a function $\mathbf{iseq:} \mathcal{C}\rightarrow (\mathcal{V}\times\mathcal{A})^\ast$.
\end{defn}

Execution of a primitive operation read or write by a user $u$ and the following state transition requires to satisfy the following information flow constraints: (i) when $u$ reads a variable $v$, information is said to flow from $v$ to $u$; therefore, should satisfy the flow constraint $\underline{v}\leqslant\underline{u}$, and (ii) when $u$ writes a variable $v$, information is said to flow from $u$ to $v$; therefore should satisfy the flow constraint $\underline{u}\leqslant\underline{v}$. In the latter case, we transfer the sensitivity of the user to the variable in order to execute the write operation if not already satisfying the constraint.

\begin{defn}[\textbf{State Transition caused by an Execution}]
In a given state $q$, the state transition function for a given command $c$ is defined as below:
\[
\delta(q,u,c) = \delta(q,u,\mathbf{iseq}(c)) = \left\{\begin{array}{ll}
								\delta(q,u,v,r) = q & \text{if }\underline{v}\leqslant\underline{u}\\
								\hspace{2cm}= \epsilon & \text{if }\underline{v}\nleqslant\underline{u}\\
								\delta(q,u,v,w) = q'[\bar{v}\leftarrow \bar{v}'] & \text{if }\underline{u}\leqslant\underline{v}\\
								\hspace{2cm}= q'[\underline{v}\leftarrow\underline{u}\oplus\underline{v},\bar{v}\leftarrow\bar{v}'] & \text{if }\underline{u}\nleqslant\underline{v}\\ 
								% \text{if }\underline{u}\nleqslant\underline{v}\quad\text{ then} & \underline{v'}=\underline{u}\oplus\underline{v}\\
								\end{array}\right\}
\]
where $\epsilon$ indicates possible violation of information flow policy. 
\end{defn}


We shall now consider an observation of a user $u$ in a given state $q$ to be defined by the function $\mathbf{view:}\mathcal{Q}\times\mathcal{U}\rightarrow\mathcal{Q}$ as below:
\[
  \begin{array}{ll}
  \textbf{view}(q,u) = q' & \text{ where } (u,v^{+})\in q' \text{ if } \underline{v}\leqslant\underline{u}\\
   & \text{ and }\hspace{4mm} (u,v^{-})\in q' \text{ if } \underline{v}\nleqslant\underline{u} \\
  \end{array}
\]
Note that the observation is subjected to the binary relation \textit{can-flow-to} over the sets $\mathcal{U}$ and $\mathcal{V}$. The function \textbf{view} says that, in a given state $q$, the value of a variable $v$ is observable (denoted by $v^{\underline{v},\bar{v}}$ or simply $v^{+}$) by the user $u$ only if $\underline{v}$ \textit{can-flow-to} $\underline{u}$; otherwise, the label and value remain concealed to the user as denoted by $v^{\varnothing,\varnothing}$ or $v^{-}$.
 
 Since the notion of non-interference demands the observation of a \textit{low} user shall remain invariant irrespective of any changes in \textit{high} inputs, we shall formally define an \textit{indistinguishable observation} in the context of our state machine.
 
 \begin{defn}[\textbf{Indistinguishable Observation}]
 For two given states $q_1$ and $q_2$, the observation of a user $u$ is said to be indistinguishable denoted by $q_1|_u\equiv q_2|_u$ iff
 \[\mathbf{view}(q_1,u)=\mathbf{view}(q_2,u)\]
 \end{defn}
 
Given a computing machine and the definition of indistinguishable observation, we now define the notion of non-interference for sequential programs.

\begin{defn}[\textbf{Non-interference for Sequential Programs}]
In a given initial state $q_0\in\mathcal{Q}$ of the computing machine $\mathcal{M}$, a sequential program $S$ is said to be non-interfering with respect to a user $u\in\mathcal{U}$ with a given label $\underline{u}$ iff $\forall s\in(\mathcal{U}\times\mathbf{iseq}(S))^\ast$ and $\forall x\in prefix-closure(s)$ the state transition $\delta(q_0,x)=q_1$ results $q_0|_u\equiv q_1|_u$.
% \[
% \forall s\in(\mathcal{U}\times\mathbf{iseq}(S))^\ast,\hspace{2mm}\forall x\in prefix-closure(s)\hspace{2mm}\lbrack (\delta(q_0,x)=q_1)\implies(q_0|_u\equiv q_1|_u)\rbrack
% \]
\end{defn}

Next, consider two programs $S_1$ and $S_2$ are executing concurrently as denoted by $S_1 \parallel S_2$. Then, the definition of non-interference must ensure that the impact of the changes in the shared variable in one program should not be observable through the variables in other programs. Let $s_1$ and $s_2$ are the input sequences issued in order to execute the programs. Then $s_1\parallel s_2$ represent a concurrent execution of the input sequences under a non-deterministic scheduler, where in each execution cycle one of the randomly chosen sequence (or a fragment) is supplied to the state machine $\mathcal{M}$. Now, the generalized definition of non-interference for the concurrent context goes as below.

\begin{defn}[\textbf{Non-interference for Concurrent Executions of Two Programs}]
\label{defn:concurrent-non-inter}
For a given machine $\mathcal{M}$, the concurrent execution of the programs $S_1$ and $S_2$ is said to be non-interfering with respect to a user $u$ with the given label $\underline{u}$ if satisfies the below conditions:
\begin{enumerate}
\item $S_1$ and $S_2$ are sequentially non-interfering with respect to the user $u$,
\item for all $x_1\in prefix-closure(s_1)$ and $x_2\in prefix-closure(s_2)$, if $\delta(q_0,t,x_1\parallel x_2)=q_1$ then $q_0|_u)\equiv q_1|_u$
\end{enumerate}
where $s_1\in(\mathcal{U}\times\mathbf{iseq}(S_1))$ and $s_2\in(\mathcal{U}\times\mathbf{seq}(S_2))$.
\end{defn}

